Electroweak corrections to monojet production at the Tevatron and the LHC

Single-jet production with missing transverse momentum is one of the most promising discovery channels for new physics at the LHC. In the Standard Model, Z + jet production with a Z-boson decay into neutrinos leads to this monojet signature. To improve the corresponding Standard Model predictions, we present the calculation of the full next-to-leading-order (NLO) electroweak corrections and a recalculation of the NLO QCD corrections to monojet production at the Tevatron and the LHC. We discuss the phenomenological impact on the total cross sections as well as on relevant differential distributions.

==> setup.tex <==
\usepackage{graphics}
%\usepackage{amsmath}
\usepackage{feynarts,slashed}
\usepackage{cite}
%\usepackage{axodraw}
\usepackage{rotating}
\usepackage{url}

\hfuzz .5pt

\makeatletter
 \setlength{\clubpenalty}{10000}
 \setlength{\widowpenalty}{10000}
 \setlength{\displaywidowpenalty}{10000}

\arraycolsep 2pt
\footnotesep 14pt

\if@twoside \oddsidemargin -17pt \evensidemargin 00pt
\else \oddsidemargin 00pt \evensidemargin 00pt
\fi
\topmargin 00pt \headheight 00pt \headsep 00pt
%\footheight 12pt \footskip 30pt
\textheight 230mm \textwidth 161mm

%\def\section{\@startsection {section}{1}{\z@}{+3.0ex plus +1ex minus
% +.2ex}{2.3ex plus .2ex}{\normalsize\bf}}
%\def\subsection{\@startsection{subsection}{2}{\z@}{+2.5ex plus +1ex
%minus +.2ex}{1.5ex plus .2ex}{\normalsize\bf}}
%\def\subsubsection{\@startsection{subsubsection}{3}{\z@}{+3.25ex plus
% +1ex minus +.2ex}{1.5ex plus .2ex}{\normalsize\bf}}

\expandafter\ifx\csname mathrm\endcsname\relax\def\mathrm#1{{\rm #1}}\fi

% Equation Numbering
\renewcommand{\theequation}{\thesection.\arabic{equation}}
\newcounter{saveeqn}
\newcommand{\alpheqn}{\setcounter{saveeqn}{\value{equation}}%
   \addtocounter{saveeqn}{1} \setcounter{equation}{0}%
   \renewcommand{\theequation}%
   {{\thesection.\arabic{saveeqn}\alph{equation}}}}
\newcommand{\reseteqn}{\setcounter{equation}{\value{saveeqn}}%
   \renewcommand{\theequation}{\thesection.\arabic{equation}}}
 
\@addtoreset{equation}{section}

\makeatother

\renewcommand{\topfraction}{0.7}
\renewcommand{\bottomfraction}{1.0}
\renewcommand{\textfraction}{0.3}
\renewcommand{\floatpagefraction}{0.7}

%\allowdisplaybreaks[3]

% new commands
\def\REF#1#2{\\[-4cm] \hspace*{#1} \rlap{\vphantom{\rule{1mm}{4cm}}
        \parbox[b]{16cm}{\baselineskip 16pt{\normalsize #2}}}}
\def\co{\relax}
\def\co{,}
\def\nl{\nonumber\\}
\def\nlc{\co\nonumber\\}
\def\nln{\nonumber\\*[-1ex]\phantom{\fbox{\rule{0em}{2ex}}}}
\def\eqskipcorr{\vspace{-\abovedisplayskip}
                \vspace{\abovedisplayshortskip}}

\def\beq{\begin{equation}}
\def\eeq{\end{equation}}
\def\beqar{\begin{eqnarray}}
\def\eeqar{\end{eqnarray}}
\def\barr#1{\begin{array}{#1}}
\def\earr{\end{array}}
\def\bfi{\begin{figure}}
\def\efi{\end{figure}}
\def\btab{\begin{table}}
\def\etab{\end{table}}
\def\bce{\begin{center}}
\def\ece{\end{center}}
\def\nn{\nonumber}
\def\disp{\displaystyle}
\def\text{\textstyle}
\def\arraystretch{1.4}


% shorthands for greek letters
\def\al{\alpha}
\def\be{\beta}
\def\ga{\gamma}
\def\de{\delta}
\def\veps{\varepsilon}
\def\la{\lambda}
\def\si{\sigma}
\def\Ga{\Gamma}
\def\De{\Delta}
\def\La{\Lambda}

% new commands for cross referencing
\def\refeq#1{\mbox{(\ref{#1})}}
\def\reffi#1{\mbox{Figure~\ref{#1}}}
\def\reffis#1{\mbox{Figures~\ref{#1}}}
%\def\refta#1{\mbox{Tab.~\ref{#1}}}
\def\refta#1{\mbox{Table~\ref{#1}}}
%\def\reftas#1{\mbox{Tabs.~\ref{#1}}}
\def\reftas#1{\mbox{Tables~\ref{#1}}}
\def\refse#1{\mbox{Section~\ref{#1}}}
\def\refses#1{\mbox{Sections~\ref{#1}}}
%\def\refse#1{\mbox{Section~\ref{#1}}}
\def\refapp#1{\mbox{App.~\ref{#1}}}
%\def\refapp#1{\mbox{Appendix~\ref{#1}}}
\def\refapps#1{\mbox{Apps.~\ref{#1}}}
\def\citere#1{\mbox{Ref.~\cite{#1}}}
\def\citeres#1{\mbox{Refs.~\cite{#1}}}

%physical units
\newcommand{\eV}{\unskip\,\mathrm{eV}}
\newcommand{\GeV}{\unskip\,\mathrm{GeV}}
\newcommand{\MeV}{\unskip\,\mathrm{MeV}}
\newcommand{\TeV}{\unskip\,\mathrm{TeV}}
\newcommand{\fba}{\unskip\,\mathrm{fb}}
\newcommand{\mba}{\unskip\,\mathrm{mb}}
\newcommand{\pba}{\unskip\,\mathrm{pb}}
\newcommand{\nba}{\unskip\,\mathrm{nb}}

%+X in processes
\newcommand{\X}{X}

%physical particles
\def\mathswitch#1{\relax\ifmmode#1\else$#1$\fi}
\def\mathswitchr#1{\relax\ifmmode{\mathrm{#1}}\else$\mathrm{#1}$\fi}
\def\mathswitchit#1{\relax\ifmmode{#1}\else$#1$\fi}
\newcommand{\PB}{\mathswitchr B}
\newcommand{\PW}{\mathswitchr W}
\newcommand{\PZ}{\mathswitchr Z}
\newcommand{\PAn}{\mathswitchr {A^0}}
\newcommand{\Pg}{\mathswitchr g}
\newcommand{\PH}{\mathswitchr H}
\newcommand{\PHgeneric}{\mathswitchr \phi^0}
\newcommand{\Pe}{\mathswitchr e}
\newcommand{\Pne}{\mathswitch \nu_{\mathrm{e}}}
\newcommand{\Pane}{\mathswitch \bar\nu_{\mathrm{e}}}
\newcommand{\Pnmu}{\mathswitch \nu_\mu}
\newcommand{\Pd}{\mathswitchr d}
%\newcommand{\Pf}{\mathswitchr f}
\newcommand{\Pf}{f}
\newcommand{\Ph}{\mathswitchr h}
\newcommand{\Pj}{\mathswitchr j}
\newcommand{\Pl}{\mathswitch l}
\newcommand{\Plp}{\mathswitch l^+}
\newcommand{\Plm}{\mathswitch l^-}
\newcommand{\Pnl}{\mathswitch {\nu_\Pl}}
\newcommand{\Pnlb}{\mathswitch {\bar{\nu}_\Pl}}
\newcommand{\Pu}{\mathswitchr u}
\newcommand{\Ps}{\mathswitchr s}
%\newcommand{\Pb}{\mathswitchr b}
\newcommand{\Pc}{\mathswitchr c}
\newcommand{\Pb}{\mathswitchr b}
\newcommand{\Pt}{\mathswitchr t}
\newcommand{\Pp}{\mathswitchr p}
\newcommand{\Ppbar}{\overline{\Pp}}
\newcommand{\Pq}{\mathswitchit q}
\newcommand{\Pep}{\mathswitchr {e^+}}
\newcommand{\Pem}{\mathswitchr {e^-}}
\newcommand{\Pepm}{\mathswitchr {e^\pm}}
\newcommand{\Pmum}{\mathswitchr {\mu^-}}
\newcommand{\PWp}{\mathswitchr {W^+}}
\newcommand{\PWm}{\mathswitchr {W^-}}
\newcommand{\PWpm}{\mathswitchr {W^\pm}}
\newcommand{\PWO}{\mathswitchr {W^0}}
\newcommand{\PZO}{\mathswitchr {Z^0}}

\newcommand{\PHu}{\mathswitchr H_\Pu}
\newcommand{\PHd}{\mathswitchr H_\Pd}
\newcommand{\Phn}{\mathswitchr {h^0}}
\newcommand{\PHn}{\mathswitchr {H^0}}

% particle masses
\newcommand{\MB}{\mathswitch {M_\PB}}
\newcommand{\Mf}{\mathswitch {m_\Pf}}
\newcommand{\Ml}{\mathswitch {m_\Pl}}
\newcommand{\Mq}{\mathswitch {m_\Pq}}
\newcommand{\MV}{\mathswitch {M_\PV}}
\newcommand{\MW}{\mathswitch {M_\PW}}
\newcommand{\hMW}{\mathswitch {\hat M_\PW}}
\newcommand{\MWpm}{\mathswitch {M_\PWpm}}
\newcommand{\MWO}{\mathswitch {M_\PWO}}
\newcommand{\MA}{\mathswitch {M_\PAn}}
\newcommand{\MZ}{\mathswitch {M_\PZ}}
\newcommand{\MH}{\mathswitch {M_\PH}}
\newcommand{\Me}{\mathswitch {m_\Pe}}
\newcommand{\Mmy}{\mathswitch {m_\mu}}
\newcommand{\Mta}{\mathswitch {m_\tau}}
\newcommand{\Md}{\mathswitch {m_\Pd}}
\newcommand{\Mu}{\mathswitch {m_\Pu}}
\newcommand{\Ms}{\mathswitch {m_\Ps}}
\newcommand{\Mc}{\mathswitch {m_\Pc}}
\newcommand{\Mb}{\mathswitch {m_\Pb}}
\newcommand{\Mt}{\mathswitch {m_\Pt}}
\newcommand{\GW}{\mathswitch {\Gamma_\PW}}
\newcommand{\GZ}{\mathswitch {\Gamma_\PZ}}

\newcommand{\Mhn}{\mathswitch {M_{\Phn}}}
\newcommand{\MHn}{\mathswitch {M_{\PHn}}}
\newcommand{\MHgeneric}{\mathswitch {M_{\PHgeneric}}}
\newcommand{\Mhntree}{\mathswitch {m_{\Phn}}}
\newcommand{\MHntree}{\mathswitch {m_{\PHn}}}

% complex masses
\newcommand{\muw}{\mathswitch {\mu_{\PW}}}

% shorthands for SM parameters
\newcommand{\scrs}{\scriptscriptstyle}
\newcommand{\sw}{\mathswitch {s_{\scrs\PW}}}
\newcommand{\cw}{\mathswitch {c_{\scrs\PW}}}
%\newcommand{\sw}{\mathswitch {s_\PW}}
%\newcommand{\cw}{\mathswitch {c_\PW}}
%\newcommand{\swbar}{\mathswitch {\bar s_\PW}}
\newcommand{\swbar}{\mathswitch {\bar s_{\scrs\PW}}}
\newcommand{\swfbar}{\mathswitch {\bar s_{\PW,\Pf}}}
\newcommand{\swqbar}{\mathswitch {\bar s_{\PW,\Pq}}}
\newcommand{\Qf}{\mathswitch {Q_\Pf}}
\newcommand{\Ql}{\mathswitch {Q_\Pl}}
\newcommand{\Qq}{\mathswitch {Q_\Pq}}
\newcommand{\vf}{\mathswitch {v_\Pf}}
\newcommand{\af}{\mathswitch {a_\Pf}}
\newcommand{\gesi}{\mathswitch {g_\Pe}^{\sigma}}
\newcommand{\gem}{\mathswitch {g_\Pe}^-}
\newcommand{\gep}{\mathswitch {g_\Pe}^+}
\newcommand{\GF}{\mathswitch {G_\mu}}
\newcommand{\Qu}{\mathswitch {Q_u}}

\newcommand{\vev}{\mathswitch v}
\newcommand{\vevu}{\mathswitch v_\Pu}
\newcommand{\vevd}{\mathswitch v_\Pd}

\newcommand{\sina}{s_\alpha}
\newcommand{\cosa}{c_\alpha}
\newcommand{\sinb}{s_\beta}
\newcommand{\cosb}{c_\beta}
\newcommand{\tana}{t_\alpha}
\newcommand{\tanb}{t_\beta}
\newcommand{\cotb}{\cot \beta}
\newcommand{\alphas}{\alpha_{\mathrm{s}}}
%\newcommand{\ptmiss}{\slashed{{p_{\mathrm{T}}}}}
\newcommand{\ptmiss}{p_{\mathrm{T}}\hspace{-1.0em}/\hspace{0.5em}}
\hyphenation{brems-strah-lung}

%various shorthands
\def\ie{i.e.\ }
\def\eg{e.g.\ }
\def\cf{cf.\ }

% slashed quantities
\newcommand{\as}{a\hspace{-0.5em}/\hspace{0.1em}}
\newcommand{\es}{\varepsilon \hspace{-0.5em}/\hspace{0.1em}}
\newcommand{\ks}{k\hspace{-0.52em}/\hspace{0.1em}}
\newcommand{\ps}{p\hspace{-0.42em}/}%\hspace{0.1em}}
\newcommand{\qs}{q\hspace{-0.5em}/\hspace{0.1em}}
\newcommand{\hb}{h\hspace{-0.5em}\vspace{-0.3em}-\hspace{0.1em}}
\marginparwidth 1.2cm

% orders of magnitude
\newcommand{\ord}{{\cal O}}
\renewcommand{\O}{{\cal O}}
%\newcommand{\C}{{\cal C}}
\newcommand{\Oa}{\mathswitch{{\cal{O}}(\alpha)}}

% various abbreviations
\newcommand{\rE}{{\mathrm{E}}}
\newcommand{\ri}{{\mathrm{i}}}
\newcommand{\re}{{\mathrm{e}}}
\newcommand{\rT}{{\mathrm{T}}}
\newcommand{\rM}{{\mathrm{M}}}
\newcommand{\ieps}{\ri\epsilon}
\newcommand{\rd}{{\mathrm{d}}}
\newcommand{\br}{{\mathrm{br}}}
\newcommand{\soft}{{\mathrm{soft}}}
\newcommand{\onel}{{\mathrm{1-loop}}}
\newcommand{\M}{{\cal {M}}}
\renewcommand{\L}{{\cal L}}
\newcommand{\F}{{\cal {F}}}
\newcommand{\bq}{{\bf q}}
\newcommand{\ehel}{\kappa}
\newcommand{\da}{\Delta\alpha}
\newcommand{\dr}{\Delta\rho}
\newcommand{\dLL}{\Delta_{\mathrm{LL}}}

\newcommand{\cut}{{\mathrm{cut}}}
\newcommand{\llog}{{\mathrm{LL}}}
\newcommand{\FSR}{{\mathrm{FSR}}}
\newcommand{\EW}{{\mathrm{EW}}}
\newcommand{\QCD}{{\mathrm{QCD}}}
\newcommand{\QED}{{\mathrm{QED}}}
\newcommand{\LEP}{{\mathrm{LEP}}}
\newcommand{\OS}{{\mathrm{OS}}}
\newcommand{\SLD}{{\mathrm{SLD}}}
\newcommand{\SM}{{\mathrm{SM}}}
\newcommand{\MSSM}{{\mathrm{MSSM}}}
\newcommand{\SUSY}{{\mathrm{SUSY}}}
\newcommand{\CM}{{\mathrm{CM}}}
\newcommand{\born}{{\mathrm{Born}}}
\newcommand{\virt}{{\mathrm{virt}}}
\newcommand{\coll}{{\mathrm{coll}}}
\newcommand{\sub}{{\mathrm{sub}}}
\newcommand{\ini}{{\mathrm{ini}}}
\newcommand{\fin}{{\mathrm{fin}}}
\newcommand{\fact}{{\mathrm{fact}}}
\newcommand{\nonfact}{{\mathrm{nonfact}}}
\newcommand{\res}{{\mathrm{res}}}
\newcommand{\rec}{{\mathrm{rec}}}
\newcommand{\PA}{{\mathrm{PA}}}
\newcommand{\real}{{\mathrm{real}}}
\newcommand{\veto}{{\mathrm{veto}}}
\newcommand{\LO}{{\mathrm{LO}}}
\newcommand{\NLO}{{\mathrm{NLO}}}
\newcommand{\Int}{{\mathrm{IF}}}
\newcommand{\full}{\mathrm{full}}


% mathematical functions
\def\atn{\mathop{\mathrm{arctan}}\nolimits}
\def\Li{\mathop{\mathrm{Li}_2}\nolimits}
\def\cLi{\mathop{{\cal L}i_2}\nolimits}
\def\Re{\mathop{\mathrm{Re}}\nolimits}
\def\Im{\mathop{\mathrm{Im}}\nolimits}
\def\sgn{\mathop{\mathrm{sgn}}\nolimits}
\def\arc{\mathop{\mathrm{arc}}\nolimits}

% Momenta
\newcommand{\pina}{\mathswitch {p_1}}
\newcommand{\Pina}{\mathswitch {p_1}}
\newcommand{\pinb}{\mathswitch {p_2}}
\newcommand{\Pinb}{\mathswitch {p_2}}
\newcommand{\knu}{\mathswitch {k_{\nu}}}
\newcommand{\Knu}{\mathswitch {k_{\nu}}}
\newcommand{\klb}{\mathswitch {k_{\Pl}}}
\newcommand{\Klb}{\mathswitch {k_{\Pl}}}
\newcommand{\kj}{\mathswitch {p_3}}
\newcommand{\Kj}{\mathswitch {p_3}}
\newcommand{\kga}{\mathswitch {k_{\ga}}}
\newcommand{\Kga}{\mathswitch {k_{\ga}}}
\newcommand{\kw}{\mathswitch {k_{\PW}}}
\newcommand{\Kw}{\mathswitch {k_{\nu}+k_{\Pl}}}

% Helicities
\newcommand{\siga}{\mathswitch {\sigma_1}}
\newcommand{\sigb}{\mathswitch {\sigma_2}}
\newcommand{\taulb}{\mathswitch {\tau_{\Pl}}}
\newcommand{\laj}{\mathswitch {\sigma_3}}
\newcommand{\laga}{\mathswitch {\lambda_{\ga}}}

% Processes
\newcommand{\udnlg}{\mathswitch {\Pu\bar{\Pd}\to\Pl^+\Pnl \mathrm{g}}}
\newcommand{\UDGG} {\mathswitch {\mathrm{gg}\Pd\Pu}}


% modifications for drafts
\newcommand{\mpar}[1]{{\marginpar{\hbadness10000%
                      \sloppy\hfuzz10pt\boldmath\bf#1}}%
                      \typeout{marginpar: #1}\ignorespaces}
\marginparwidth 1.2cm
\marginparsep 0.2cm
\def\draftdate{\relax}
\def\mda{\relax}
\def\mua{\relax}
\def\mla{\relax}
\def\draft{
\def\thtystars{******************************}
\def\sixtystars{\thtystars\thtystars}
\typeout{}
\typeout{\sixtystars**}
\typeout{* Draft mode!
         For final version remove \protect\draft\space in source file *}
\typeout{\sixtystars**}
\typeout{}
\def\draftdate{\today}
\def\mua{\marginpar[\boldmath\hfil$\uparrow$]%
                   {\boldmath$\uparrow$\hfil}%
                    \typeout{marginpar: $\uparrow$}\ignorespaces}
\def\mda{\marginpar[\boldmath\hfil$\downarrow$]%
                   {\boldmath$\downarrow$\hfil}%
                    \typeout{marginpar: $\downarrow$}\ignorespaces}
\def\mla{\marginpar[\boldmath\hfil$\rightarrow$]%
                   {\boldmath$\leftarrow $\hfil}%
                    \typeout{marginpar: $\leftrightarrow$}\ignorespaces}
\def\Mua{\marginpar[\boldmath\hfil$\Uparrow$]%
                   {\boldmath$\Uparrow$\hfil}%
                    \typeout{marginpar: $\Uparrow$}\ignorespaces}
\def\Mda{\marginpar[\boldmath\hfil$\Downarrow$]%
                   {\boldmath$\Downarrow$\hfil}%
                    \typeout{marginpar: $\Downarrow$}\ignorespaces}
\def\Mla{\marginpar[\boldmath\hfil$\Rightarrow$]%
                   {\boldmath$\Leftarrow $\hfil}%
                    \typeout{marginpar: $\Leftrightarrow$}\ignorespaces}
\overfullrule 5pt
\oddsidemargin -15mm
\marginparwidth 29mm
}

% change of eqnarray environment
%  Default is for left-hand side of equations to be flushleft.
%  To make them flushright, \let\@eqnsel = \hfil

\makeatletter
%\let\@eqnsel = \hfil

\def\eqnarray{\stepcounter{equation}\let\@currentlabel=\theequation
\global\@eqnswtrue
\global\@eqcnt\z@\tabskip\@centering\let\\=\@eqncr
%$$\halign to \displaywidth\bgroup\@eqnsel\hskip\@centering
%  $\displaystyle\tabskip\z@{##}$&\global\@eqcnt\@ne
$$\halign to \displaywidth\bgroup\hskip\@centering
  $\displaystyle\tabskip\z@{##}$\@eqnsel&\global\@eqcnt\@ne
  \hskip 2\arraycolsep \hfil${##}$\hfil
  &\global\@eqcnt\tw@ \hskip 2\arraycolsep $\displaystyle\tabskip\z@{##}$\hfil
   \tabskip\@centering&\llap{##}\tabskip\z@\cr}
\def\appendix{\par
 \setcounter{section}{0} \setcounter{subsection}{0}
 \def\thesection{\Alph{section}}}

\newcommand{\gtrless}
{\;\rlap{\raisebox{+.25em}{$>$}}\raisebox{-.25em}{$<$}\;}
\newcommand{\lsim}
{\;\raisebox{-.3em}{$\stackrel{\displaystyle <}{\sim}$}\;}
\newcommand{\gsim}
{\;\raisebox{-.3em}{$\stackrel{\displaystyle >}{\sim}$}\;}
\def\asymp#1{\;\raisebox{-.4em}{$\widetilde{\scriptstyle #1}$}\;}
\newcommand{\gl}
{\;\raisebox{.25em}{$>$}\hspace{-.75em}\raisebox{-.2em}{$<$}\;}
\def\dsl{\mathpalette\make@slash}
\def\make@slash#1#2{\setbox\z@\hbox{$#1#2$}%
  \hbox to 0pt{\hss$#1/$\hss\kern-\wd0}\box0}

\newcommand{\mycaption}[2][]{{\begin{center} \parbox{15cm}{{\bf \caption[#1]{\rm {#2}}}} \end{center} }}
%\newcommand{\mycaption}[2][kurz]{{{\bf \caption[#1]{\rm {#2}}}}}

\newcommand{\Vector}[1]{{\left( \begin{array}{c} #1 \end{array} \right) }}
\newcommand{\Matrix}[1]{{\left( \begin{array}{cc} #1 \end{array} \right) }}
\newcommand{\mr}[1]{{\mathrm{#1}}}
\renewcommand{\la}{{\mathcal L}}
\newcommand{\Pbbar}{{\bar{\Pb}}}
\newcommand{\Pdbar}{{\bar{\Pd}}}
\newcommand{\Pubar}{{\bar{\Pu}}}
\newcommand{\Pqbar}{{\bar{\Pq}}}
\newcommand{\MSbar}{{$\overline{\mathrm{MS}}$}}
\newcommand{\DRbar}{{$\overline{\mathrm{DR}}$}}

\newcommand{\comment}[1]{{\noindent {\bf (#1)}}}

\newcommand{\myplot}[9]{
\begin{picture}(0,0)(0,0)
\put(#2,#3){#4}
\begin{rotate}{#8}
\put(#5,#6){#7}
\end{rotate}
\end{picture}
\includegraphics[width=#9]{#1}
}

\newcommand{\RL}{\mathrm{L}}
\newcommand{\RT}{\mathrm{T}}

\makeatother

\def\sub{{\mathrm{sub}}}
\def\sli{{\mathrm{sli}}}
\def\gsub{g^{(\sub)}}
\def\hsub{h}
\def\Gsub{G^{(\sub)}}
\def\Gsli{G^{(\sli)}}
\def\Hsub{H}
\def\cGsub{{\cal G}^{(\sub)}}
\def\cHsub{{\cal H}}
\def\cHsli{{\cal H}}
\def\bcGsub{\bar {\cal G}^{(\sub)}}
\def\bcGsli{\bar {\cal G}^{(\sli)}}
\def\bcHsub{\bar {\cal H}}
\def\ssub{\sigma^{(\sub)}}
\def\gin{g^{\mathrm{(in)}}}
\def\gout{g^{\mathrm{(out)}}}
\def\goutin{g^{\mathrm{(out/in)}}}

\newcommand{\phz}{\phantom{(0)}}

